A coupled model for the linked dynamics of marine pollution by microplastics and plastic-related organic pollutants

The pervasiveness of microplastics in global oceans is raising concern about its impacts on organisms. While quantifying its toxicity is still an open issue, sampling evidence has shown that rarely is marine microplastics found clean; rather, it is often contaminated by other types of chemical pollutants, some known to be harmful to biota and humans. To provide a first tool for assessing the role of microplastics as vectors of plastic-related organic pollutants (PROPs), we developed a data-informed model that accounts for the intertwined dynamics of Lagrangian microplastic particles transported by surface currents and the Eulerian advection-diffusion of chemicals that partition on them through seawater-particle interaction. Focusing on the Mediterranean Sea and using simple, yet realistic forcings for the input of PROPs, our simulations highlight that microplastics can mediate PROP export across different sub-seas. Particle origin, in terms of both source type (either coastal, riverine, or fishing-derived) and geographical location, seems to play a major role in determining the amount of PROPs conveyed by microplastics during their journey at sea. We argue that quantitative numerical modelling approaches can be focal to shed some light on the vast spatial and temporal scales of microplastics-PROPs interaction, complementary to much-needed on-field investigation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
